Robust Ensemble Model Training via Random Layer Sampling Against Adversarial Attack

Deep neural networks have achieved substantial achievements in several computer vision areas, but have vulnerabilities that are often fooled by adversarial examples that are not recognized by humans. This is an important issue for security or medical applications. In this paper, we propose an ensemble model training framework with random layer sampling to improve the robustness of deep neural networks. In the proposed training framework, we generate various sampled model through the random layer sampling and update the weight of the sampled model. After the ensemble models are trained, it can hide the gradient efficiently and avoid the gradient-based attack by the random layer sampling method. To evaluate our proposed method, comprehensive and comparative experiments have been conducted on three datasets. Experimental results show that the proposed method improves the adversarial robustness.

==> Section/Acknowledgements.tex <==
This work was conducted by Center for Applied Research in Artificial Intelligence (CARAI) grant funded by DAPA and ADD (UD190031RD).

==> Section/Related_Work.tex <==
\subsection{Adversarial Attack Method}
The deep neural networks have been shown to be highly vulnerable to adversarial examples. It was first discovered by Szegedy et al. \cite{szegedy2013intriguing}. Then, Goodfellow et al. \cite{goodfellow2014explaining} proposed Fast Gradient Sign Method (FGSM). It is a fast and single-step adversarial attack version of \cite{szegedy2013intriguing}. It performs a single step update on the original sample $x$ along the direction of the gradient of a loss function. After that, Moosavi et al. designed the DeepFool attack \cite{moosavi2016deepfool} starting from the assumption that models are fully linear. Under this assumption, there is a polyhedron that can separate individual classes. Recently, more powerful and effective attacks including C\&W \cite{carlini2017towards}, PGD \cite{madry2018towards}, EAD \cite{chen2018ead} are proposed to fool the networks. As stronger attack methods are reported, the need for developing better defense methods is increased.
\subsection{Adversarial Defense Method}
To improve the model’s robustness against adversarial examples, several methods have been reported. There are many approaches including distillation-based approaches \cite{papernot2016distillation}, adversarial training approaches \cite{madry2018towards, athalye2018obfuscated}, and ensemble training approaches \cite{lakshminarayanan2017simple, pang2019improving, liu2018towards, dhillon2018stochastic}. In this section, we mainly describe the ensemble training approaches.

Pang et al. \cite{pang2019improving} improves the adversarial robustness by promoting ensemble diversity with Adaptive Diversity Promoting (ADP) regularization. They trained ensemble model through ADP regularization method. Through the ensemble diversity, the non-maximal predictions of each model are mutually orthogonal, then predicts robust output. Smith et al. \cite{smith2018understanding} proposed ensemble models training method with predictive uncertainty estimation and detecting adversarial example. By quantifying the predictive uncertainty, they could optimize the ensemble models that are robust to adversarial examples. It could also detect adversarial examples with predictive uncertainty. Although these ensemble model training methods could improve the adversarial robustness, to improve the adversarial robustness, a large number of parameters are required. Another way to construct ensemble models is to add the noise in the layer or dropout the weight. The noise addition or dropout method can be interpreted as ensemble model combination \cite{lakshminarayanan2017simple} where the predictions are averaged over an ensemble of neurons. Liu et al. \cite{liu2018towards} reported a random self-ensemble (RSE) training for improving the robustness of deep neural models. They add a noise layer before each convolution layer in both training and prediction phases. They showed that the algorithm is equivalent to ensemble a huge amount of noisy models together, and ensure that the ensemble model can generalize well. They further prove the fact that the proposed method is equivalent to adding a Lipchitz regularization and thus can improve the robustness of neural models. Dhillon et al. \cite{dhillon2018stochastic} proposed stochastic activation pruning for robust adversarial defense. During the forward pass, they prune a subset of the activations in each layer. Then, they scale up the remaining activations to normalize the dynamic range of the inputs to the subsequent layer.
